NARUTO: Neural Active Reconstruction from Uncertain Target Observations

We present NARUTO, a neural active reconstruction system that combines a hybrid neural representation with uncertainty learning, enabling high-fidelity surface reconstruction. Our approach leverages a multi-resolution hash-grid as the mapping backbone, chosen for its exceptional convergence speed and capacity to capture high-frequency local features.The centerpiece of our work is the incorporation of an uncertainty learning module that dynamically quantifies reconstruction uncertainty while actively reconstructing the environment. By harnessing learned uncertainty, we propose a novel uncertainty aggregation strategy for goal searching and efficient path planning. Our system autonomously explores by targeting uncertain observations and reconstructs environments with remarkable completeness and fidelity. We also demonstrate the utility of this uncertainty-aware approach by enhancing SOTA neural SLAM systems through an active ray sampling strategy. Extensive evaluations of NARUTO in various environments, using an indoor scene simulator, confirm its superior performance and state-of-the-art status in active reconstruction, as evidenced by its impressive results on benchmark datasets like Replica and MP3D.

==> alg_fig_table/tab_replica_results_occ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% w/ culling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
    \centering
    \begin{tabular}{|c|l*{8}{c}|c|}
        \hline
        Method &  & 
        office0 & office1 & office2 & office3 & office4 & room0 & room1 & room2 & 
        Avg. \\
        \cline{3-10}
        \hline

        % Co-SLAM
        \multirow{3}{*}{\makecell{Co-SLAM \\ (w/o tracking)}} 
        % & Depth L1 [cm] $\downarrow$ & 1.05 & 0.85 & 2.37 & 1.24 & 1.48 & 1.86 & 1.66 & 1.54 & 1.51 \\
        & Acc. [cm] $\downarrow$ & 1.42 & 1.11 & 1.68 & 2.02 & 1.80 & 1.66 & 1.32 & 1.60  & 1.58 \\
        & Comp. [cm] $\downarrow$ & 1.40 & 1.17 & 1.61 & 1.86 & 1.72 & 1.59 & 1.31 & 1.56 & 1.53 \\
        & Comp. Ratio $\uparrow$ & 98.00 & 98.18 & 98.34 & 97.49 & 97.96 & 99.25 & 99.28 & 97.53 & 98.25 \\
        \hline

        % ActiveRay
        \multirow{3}{*}{Ours (ActiveRay)} 
        % & Depth L1 (cm) & & & & & & & & & \\
        & Acc. (cm) $\downarrow$ & 1.39 & 1.10 & 1.64 & 2.04 & 1.80 & 1.65 & 1.31 & 1.58 & 1.56 \\
        & Comp. (cm) $\downarrow$ & 1.39 & 1.17 & 1.59 & 1.85 & 1.71 & 1.59 & 1.31 & 1.55 & 1.52 \\
        & Comp. Ratio $\uparrow$ & 98.07 & 98.19 & 98.49 & 97.51 & 98.04 & 99.27 & 99.27 & 97.63 & 98.31 \\
        \hline

        % ActivePlan
        \multirow{3}{*}{Ours (ActivePlan)} 
        % & Depth L1 (cm) & & & & & & & & & \\
        & Acc. (cm) $\downarrow$ &
        1.34 & 1.12 & 1.56 & 1.95 & 1.67 & 1.56 & 1.26 & 1.42 & 1.49 \\
        & Comp. (cm) $\downarrow$ & 
        1.32 & 1.13 & 1.57 & 2.03 & 1.68 & 1.56 & 1.29 & 1.43 & 1.50 \\
        & Comp. Ratio $\uparrow$ & 
        99.08 & 99.00 & 99.34 & 97.14 & 98.91 & 99.63 & 99.53 & 99.12 & 98.97 \\
        \hline

        % Full
        \multirow{3}{*}{Ours (Full)} 
        % & Depth L1 (cm) & & & & & & & & & \\
        & Acc. (cm) $\downarrow$ & 
        1.33 & 1.12 & 1.58 & 1.91 & 1.70 & 1.57 & 1.26 & 1.43 & 1.49 \\
        & Comp. (cm) $\downarrow$ & 
        1.32 & 1.13 & 1.58 & 1.82 & 1.69 & 1.56 & 1.26 & 1.43 & 1.47 \\
        & Comp. Ratio $\uparrow$ & 
        99.08 & 98.81 & 99.22 & 98.43 & 98.85 & 99.65 & 99.59 & 99.08 & 99.09\\
        \hline
    \end{tabular}
    \caption{Replica Results: with occlusion mask}
\end{table*}


==> others/rrt.tex <==
import numpy as np
import matplotlib.pyplot as plt

class Node:
    def __init__(self, x, y, z):
        self.x = x
        self.y = y
        self.z = z
        self.parent = None

class RRT:
    def __init__(self, start, goal, sdf_map, max_samples=200, step_size=0.5, maxz=None):
        self.start = Node(*start)
        self.goal = Node(*goal)
        self.sdf_map = sdf_map
        margin = 0
        self.x_range = [margin, self.sdf_map.shape[0] - 1 - margin]  # safe margin from boundary
        self.y_range = [margin, self.sdf_map.shape[1] - 1 - margin]
        self.z_range = [margin, min(self.sdf_map.shape[2] - 1 - margin, maxz)]
        self.max_samples = max_samples
        self.step_size = step_size
        ### HY-006: RRT nodes here. each node has a parent, and it can form the full tree ###
        self.nodes = [self.start] 

    def generate_random_point(self):
        x = np.random.uniform(self.x_range[0], self.x_range[1])
        y = np.random.uniform(self.y_range[0], self.y_range[1])
        z = np.random.uniform(self.z_range[0], self.z_range[1])
        return x, y, z

    def find_nearest_node(self, point):
        distances = [(node.x - point[0])**2 + (node.y - point[1])**2 + (node.z - point[2])**2 for node in self.nodes]
        nearest_node_index = distances.index(min(distances))
        return self.nodes[nearest_node_index]

    def is_collision_free(self, node1, node2):
        pa = np.array([node1.x, node1.y, node1.z])
        pb = np.array([node2.x, node2.y, node2.z])
        points = np.linspace(pa, pb, num=int(np.ceil(np.linalg.norm(pb - pa) / (self.step_size / 5))) + 1)
        points = np.round(points, decimals=0)
        points = points.astype(int)
        
        collision_free = self.sdf_map[points[:,0], points[:,1], points[:,2]].min() >= 0.4
        # collision_free = collision_free and self.sdf_map[int(node1.x), int(node1.y), int(node1.z)] >= 0
        
        if collision_free and self.sdf_map[round(node2.x), round(node2.y), round(node2.z)] < 0:
            breakpoint()
        
        return collision_free

    def extend_tree(self):
        random_point = self.generate_random_point()
        nearest_node = self.find_nearest_node(random_point)
        x_diff = random_point[0] - nearest_node.x
        y_diff = random_point[1] - nearest_node.y
        z_diff = random_point[2] - nearest_node.z
        distance = np.linalg.norm([x_diff, y_diff, z_diff])
        if distance > self.step_size:
            x_new = nearest_node.x + (x_diff / distance) * self.step_size
            y_new = nearest_node.y + (y_diff / distance) * self.step_size
            z_new = nearest_node.z + (z_diff / distance) * self.step_size
        else:
            x_new = random_point[0]
            y_new = random_point[1]
            z_new = random_point[2]
        new_node = Node(x_new, y_new, z_new)
        if self.is_collision_free(nearest_node, new_node):
            new_node.parent = nearest_node
            self.nodes.append(new_node)

    def run(self):
        ### RRT planning ###
        for _ in range(self.max_samples):
            self.extend_tree()
            if np.linalg.norm([self.nodes[-1].x - self.goal.x, self.nodes[-1].y - self.goal.y, self.nodes[-1].z - self.goal.z]) < self.step_size:
                print(f"[DEBUG] | RRT | Early break RRT planning")
                break
                
        ### check if RRT sucess ###
        last = self.find_nearest_node([self.goal.x, self.goal.y, self.goal.z])
        dist_last2goal = np.linalg.norm(np.array([last.x-self.goal.x, last.y-self.goal.y, last.z-self.goal.z]))
        # if dist_last2goal > self.step_size:
        #     return False
        # if np.array
        if self.sdf_map[round(last.x), round(last.y), round(last.z)] < 0:
            print("Goal is not reachable !!!!!!!!!!!!!!!!!!!!")
        self.goal.parent = last
        # return True

    def find_path(self):
        path = [self.goal]
        current_node = self.goal
        while current_node.parent is not None:
            path.append(current_node.parent)
            current_node = current_node.parent
        return path

# Example usage
if __name__ == "__main__":
    # Create a 3D occupancy grid map (0 for free space, 1 for obstacles)
    occupancy_map = np.zeros((100, 100, 100), dtype=int)
    occupancy_map[50:80, 50:80, 50:80] = 1

    # Define the start and goal points
    start_point = (10, 10, 10)
    goal_point = (90, 90, 90)

    # Define the environment boundaries
    x_range = (0, 100)
    y_range = (0, 100)
    z_range = (0, 100)

    # Initialize RRT and find the path
    rrt = RRT(start_point, goal_point, occupancy_map, x_range, y_range, z_range)
    rrt.run()
    path = rrt.find_path()

    # Visualize the path (plotting only the x and y coordinates)
    path_x = [node.x for node in path]
    path_y = [node.y for node in path]
    plt.plot(path_x, path_y, 'r-', linewidth=2)
    plt.plot(start_point[0], start_point[1], 'go', markersize=8)
    plt.plot(goal_point[0], goal_point[1], 'ro', markersize=8)
    plt.xlabel('X')
    plt.ylabel('Y')
    plt.title('RRT Path Planning in 2D')
    plt.grid(True)
    plt.show()


==> others/rrt_connect.tex <==
import numpy as np
import matplotlib.pyplot as plt

class Node:
    def __init__(self, x, y, z):
        self.x = x
        self.y = y
        self.z = z
        self.parent = None

class RRT:
    def __init__(self, start, goal, sdf_map, max_samples=200, step_size=0.5, maxz=None):
        self.start = Node(*start)
        self.goal = Node(*goal)
        self.sdf_map = sdf_map
        margin = 0
        self.x_range = [margin, self.sdf_map.shape[0] - 1 - margin]  # safe margin from boundary
        self.y_range = [margin, self.sdf_map.shape[1] - 1 - margin]
        self.z_range = [margin, min(self.sdf_map.shape[2] - 1 - margin, maxz)]
        self.max_samples = max_samples
        self.step_size = step_size
        ### HY-006: RRT nodes here. each node has a parent, and it can form the full tree ###
        self.nodes = [self.start, self.goal]
        self.start_tree = [self.start]
        self.goal_tree = [self.goal]
        self.intersection = []

    def generate_random_point(self):
        x = np.random.uniform(self.x_range[0], self.x_range[1])
        y = np.random.uniform(self.y_range[0], self.y_range[1])
        z = np.random.uniform(self.z_range[0], self.z_range[1])
        return x, y, z

    def find_nearest_node(self, point, tree):
        distances = [(node.x - point[0])**2 + (node.y - point[1])**2 + (node.z - point[2])**2 for node in tree]
        nearest_node_index = distances.index(min(distances))
        return tree[nearest_node_index]

    def is_collision_free(self, node1, node2):
        pa = np.array([node1.x, node1.y, node1.z])
        pb = np.array([node2.x, node2.y, node2.z])
        points = np.linspace(pa, pb, num=int(np.ceil(np.linalg.norm(pb - pa) / (self.step_size / 5))) + 1)
        points = np.round(points, decimals=0)
        points = points.astype(int)
        
        collision_free = self.sdf_map[points[:,0], points[:,1], points[:,2]].min() >= 0.4
        # collision_free = collision_free and self.sdf_map[int(node1.x), int(node1.y), int(node1.z)] >= 0
        
        if collision_free and self.sdf_map[round(node2.x), round(node2.y), round(node2.z)] < 0:
            breakpoint()
        
        return collision_free

    def extend_tree(self):
        random_point = self.generate_random_point()
        nearest_node = self.find_nearest_node(random_point, self.nodes)
        x_diff = random_point[0] - nearest_node.x
        y_diff = random_point[1] - nearest_node.y
        z_diff = random_point[2] - nearest_node.z
        distance = np.linalg.norm([x_diff, y_diff, z_diff])
        if distance > self.step_size:
            x_new = nearest_node.x + (x_diff / distance) * self.step_size
            y_new = nearest_node.y + (y_diff / distance) * self.step_size
            z_new = nearest_node.z + (z_diff / distance) * self.step_size
        else:
            x_new = random_point[0]
            y_new = random_point[1]
            z_new = random_point[2]
        new_node = Node(x_new, y_new, z_new)
        dist_2_goal = 9999
        nearest_goal = None
        if self.is_collision_free(nearest_node, new_node):
            new_node.parent = nearest_node
            if nearest_node in self.start_tree:
                self.start_tree.append(new_node)
                nearest_goal = self.find_nearest_node([new_node.x, new_node.y, new_node.z], self.goal_tree)
            else:
                self.goal_tree.append(new_node)
                nearest_goal = self.find_nearest_node([new_node.x, new_node.y, new_node.z], self.start_tree)
            
            dist_2_goal = np.linalg.norm([new_node.x - nearest_goal.x, new_node.y - nearest_goal.y, new_node.z - nearest_goal.z])
            self.nodes.append(new_node)
        return dist_2_goal, new_node, nearest_goal

    def run(self):
        ### RRT planning ###
        for step in range(self.max_samples):
            dist2goal, new_node, nearest_goal = self.extend_tree()
            if dist2goal < self.step_size:
                print(f"[DEBUG] | RRT | Early break RRT planning")
                print(step)
                self.intersection += [new_node, nearest_goal]
                return True
        print("Goal is not reachable !!!!!!!!!!!!!!!!!!!!")
        return False

    def find_path(self):
        start_path = []
        goal_path = []
        for intersect in self.intersection:
            if intersect in self.start_tree:
                start_path.append(intersect)
                while start_path[-1].parent is not None:
                    start_path.append(start_path[-1].parent)
                start_path = start_path[::-1]
            elif intersect in self.goal_tree:
                goal_path.append(intersect)
                while goal_path[-1].parent is not None:
                    goal_path.append(goal_path[-1].parent)
        print(len(start_path), len(goal_path))
        return start_path + goal_path

# Example usage
if __name__ == "__main__":
    # Create a 3D occupancy grid map (0 for free space, 1 for obstacles)
    occupancy_map = np.ones((100, 100, 20), dtype=int)
    occupancy_map[50:80, 50:80, 5:10] = 0

    # Define the start and goal points
    start_point = (10, 10, 10)
    goal_point = (90, 90, 19)


    # Initialize RRT and find the path
    rrt = RRT(start_point, goal_point, occupancy_map, max_samples=40000, step_size=2, maxz=100)
    rrt.run()
    path = rrt.find_path()

    # Visualize the path (plotting only the x and y coordinates)
    path_x = [node.x for node in path]
    path_y = [node.y for node in path]
    plt.plot(path_x, path_y, 'r-', linewidth=2)
    plt.plot(start_point[0], start_point[1], 'go', markersize=8)
    plt.plot(goal_point[0], goal_point[1], 'ro', markersize=8)
    plt.plot(rrt.intersection[0].x, rrt.intersection[0].y, 'bo', markersize=8)
    plt.xlabel('X')
    plt.ylabel('Y')
    plt.title('RRT Path Planning in 2D')
    plt.grid(True)
    plt.show()


==> sec/3_preliminaries.tex <==
\section{Preliminaries: Neural 3D Reconstruction}
\label{sec:preliminaries}

In this section, we provide preliminaries for the neural mapping module. 
Given a stream of observations (RGB-D images) with known camera intrinsics, 
dense mapping can be performed by optimizing a neural scene representation where a variety of representations can be adopted, e.g. radiance field, occupancy map, or truncated signed distance (TSDF). 
For 3D reconstruction, TSDF is a commonly used representation. 
Recently, neural implicit representations have been proven to have impressive expressiveness and compactness that encode the appearance and 3D geometry of the scene. 

